DRAPS: Dynamic and Resource-Aware Placement Scheme for Docker Containers in a Heterogeneous Cluster

Virtualization is a promising technology that has facilitated cloud computing to become the next wave of the Internet revolution. Adopted by data centers, millions of applications that are powered by various virtual machines improve the quality of services. Although virtual machines are well-isolated among each other, they suffer from redundant boot volumes and slow provisioning time. To address limitations, containers were born to deploy and run distributed applications without launching entire virtual machines. As a dominant player, Docker is an open-source implementation of container technology. When managing a cluster of Docker containers, the management tool, Swarmkit, does not take the heterogeneities in both physical nodes and virtualized containers into consideration. The heterogeneity lies in the fact that different nodes in the cluster may have various configurations, concerning resource types and availabilities, etc., and the demands generated by services are varied, such as CPU-intensive (e.g. Clustering services) as well as memory-intensive (e.g. Web services). In this paper, we target on investigating the Docker container cluster and developed, DRAPS, a resource-aware placement scheme to boost the system performance in a heterogeneous cluster.

==> solution__Ying_Mao_s_conflicted_copy_2017-07-13_.tex <==
\section{\sol~ in a Heterogeneous Cluster}
Previously, we discuss the different modules in \sol~ and their major responsibilities. 
In this section, we present the detailed design of \sol~, in a heterogeneous cluster, 
which aims to increase resource availability on each worker node and boost the service performance.
To achieve the objectives, \sol~ system consists of three strategics, 
%1) Understand the dynamic resource demand of Docker container 
1) Identify dominate resource demands of containers;
2) Initial container placement; 
3) Migrate a container



\begin{figure*}[ht]
%\hspace*{0.8in}
   \centering
%\vspace{-0.1in}
      \begin{subfigure}[t]{0.24\linewidth}
\centering
      \includegraphics[width=\linewidth]{cpu}
      \vspace{-0.15in}
      \caption{Usage of CPU}
      \label{fig:cpu}
      \end{subfigure} %
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \begin{subfigure}[t]{0.24\linewidth}
\centering
      \includegraphics[width=\linewidth]{mem}
      \vspace{-0.15in}
      \caption{Usage of Memory}
      \label{fig:mem}
      \end{subfigure} %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
      \begin{subfigure}[t]{0.24\linewidth}
\centering
      \includegraphics[width=\linewidth]{netio}
      \vspace{-0.15in}
      \caption{Usage of Network I/O}
      \label{fig:netio}
      \end{subfigure} %
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \begin{subfigure}[t]{0.24\linewidth}
\centering
      \includegraphics[width=\linewidth]{blockio}
      \vspace{-0.15in}
      \caption{Usage of Block I/O}
      \label{fig:blockio}
      \end{subfigure} %
\caption{Resource demonds under different workloads on four services, MySQL, Tomcat, YUM, PI.}
\end{figure*}

\subsection{Identify Resource Demands of Containers}
\label{understand}
Before improving the overall resource efficiency, the system needs to understand the dynamic resource demand of various containers. 
A container is, usually, focused on providing a specific service, such as web browsing, data sorting, and database querying. 
Different algorithms and operations will be applied to the services, which result in a diverse resource demands.
As an intuitive example, we conduct the experiments on NSF Cloudlab~\cite{cloudlab} (M400 node hosted by University of Utah).
The containers are initiated by using the following four images and the data is collected through ``docker stats'' command.
\begin{enumerate}
 \item MySQL: the relational database management system. Tested workloads: scan, select, count, join.
 \item Tomcat: provides HTTP web services with Java. Tested workloads: HTTP queries at 10/second and 20/second of a HelloWorld webpage.
 \item YUM: a software package manager that installs, updates, and removes packages. Tested workload: download and install ``vim'' package. 
 \item PI: a service to calculate PI. Tested workload: top 3,000 digits with single thread, top 7,500 digits with two threads.
\end{enumerate}  
\cref{fig:cpu,fig:mem,fig:netio,fig:blockio} plots the dynamic resource demands under different workloads on the above four Docker containers.
The figures illustrate very diverse usage patterns on four types of resources, CPU, memory, network I/O and block I/O.
For example, without workload, container PI consumes very limited resources. However, when the jobs arrive at 10th and 38th second, the CPU usage
jumps to 100\% for a single thread job and 200\% for a two-threads job. The usages of the other three types of resources still remain at very low level.
For MySQL service container, with tested operations, the CPU usage shows a burst when client submit a request. At time 84, a ``join'' operation that involves
3 tables is submitted, we can find CPU usage jumps as well as memory usage. The reason is that join operation needs lots of computation and copies
of tables in memory. Different usage trends are found on YUM and Tomcat services, where YUM uses less CPU and memory, but more network I/O and block I/O to
download and install packages. On the other hand,
Tomcat consumes a very small amount of network I/O and block I/O due the size of a tested HelloWorld page, but more than 200MB memory is used to maintain the 
service. 


To balance the resource usage, it's crucial to place the containers with complementary demands on the same worker, 
As shown on the graphs, despite multiple types of resources, 
there is a dominate resource demand of a service in a given period. 

In DRAP, we need to identify the a dominate resource demand for each service. 
A manager, in the system, can monitor all containers' resource usage and group them by their associated service ID. 
Suppose the service $s_i \in S$ contains
$m$ running containers that store in a set, $RC_{s_i}$. The resources consumed by $c_i \in RC_{s_i}$ is denoted by a vector, 
$R_{c_i}$, where each attribute, $r_i$, in the vector represents a type of resources, such as memory and CPU. 
If there are $q$ types of resources in the system, the average resource cost of $s_i$ is a vector, $R_{s_i}$,
\begin{equation*}
\begin{aligned}
 R_{s_i} & = \sum\nolimits_{c_i \in RC_{s_i}} R_{c_i} \\
         & = <\sum_{c_i \in RC_{s_i}} r_1 / m, \sum_{c_i \in RC_{s_i}} r_2 / m, ..., \sum_{c_i \in RC_{s_i}} r_q / m>
 \end{aligned}
\end{equation*}

On the worker nodes, there is a limited amount of resources in each type. 
The resource limit is a vector that contains $q$ attributes, $<l_1, l_2, ..., l_q>$. 
The limit of a system, $<L_1, L_2, ..., L_q>$, is obtained by sum up the the vectors from workers.
Therefore,  $R_{s_i}$ can be represented by a percent of total resources in the system, for the 
$i^{th}$ type, the container cost for $s_i$ in average is $\sum_{c_i \in RC_{s_i}} r_i / m \div L_i$.
With the analysis, we define the dominate function, 
\begin{equation*}
  DOM(s_i) = max \{ \sum_{c_i \in RC_{s_i}} r_i / m \div L_i \}
\end{equation*}
Function $DOM(s_i)$ returns the type of a dominate resource demand of service $s_i$ within a given time period.
Depending on the running containers for $s_i$ and the current cost of them, the value of $DOM(s_i)$ changes along with
system goes.


\subsection{Initial Container Placement}
To use a Swarmkit cluster, clients need to execute a ``docker run'' command to start a new container.
Therefore, the first task for the cluster is to choose a worker node to host the container.
As discussed in section~\ref{back}, the default container placement strategy fails to take dynamic 
resource contention into consideration. It is because that the managers in Swarmkit 
do not have a mechanism to monitor the current available resource. 
\sol, on the other hand, addresses the problem by introducing DRAP-Heartbeat.
DRAP-Heartbeat is an enhanced heartbeat message that not only the states of worker node, but also the
containers' resource usage over a given time window, the usage includes, memory, cpu, bandwidth, and block i/o.
At the manager side, the data will be organized into a table that keep tracking the current available resource 
on each worker and its corresponding containers' resource usages.

Running on managers, Algorithm~\ref{alg:initial} assigns a container initialization task to a specific worker.
Firstly, each manager maintains a known service set that records dockers' characteristics, such as the usage of memory, CPU, bandwidth, and block i/o (line 1).
The initial candidate worker are all running workers (line 2).
When a starting new container task arrives, the algorithm applies all filters that user specified to shrink the candidate work set, $W_{cand}$ (line 3-6).
Then, it checks whether the container belongs to a known service (line 7). If it is, the $S_{dom}$ parameter will be used to store the container's dominate 
resource attribute (line 8). In \sol, we consider four types, memory, CPU, bandwidth, and block i/o.
The $W_{cand}$ set will be sorted according to the dominate resource attribute and 
return the $W_{id}$ with highest available resource in $S_{dom}$ type (line 9-10).
If the service cannot be found in $\{KS\}$, $W_{id}$ with the highest available resource in average will be chosen (line 11-13).

\begin{algorithm}[ht]
\begin{algorithmic}[1]
\STATE Maintains a known characteristics service set $\{KS\}$ 
%and a table that records the current available resource $\{AR\}$;
\STATE $\{W_{cand}\}$ = All running $W_{id}$;
\STATE {\bf Function ContainerPlacement($S_{ID}$)}

\FOR {$w_{id} \in \{W_{cand}\}$}
\IF {$!Filters(w_{id})$}
\STATE Remove $w_{id}$ from $\{W_{cand}\}$
\ENDIF
\ENDFOR

\IF {$S_{ID} \in \{KS\}$}
\STATE $S_{DOM} =  DOM(S_{ID})$
\STATE Sort $W_{cand}$ according to $r_{S_{DOM}}$
\STATE Return $w_{id}$ with highest $r_{S_{DOM}}$

\begin{comment}
  \IF {$S_{dom} = ``M''$}
  \STATE Sort $\{W_{cand}\}$ according to $W_{mem}$
  \STATE Return $W_{id}$ with highest $W_{mem}$
  
  \ELSIF {$S_{DOM} = ``C''$}
  \STATE Sort $\{W_{cand}\}$ according to $W_{cpu}$
  \STATE Return $W_{id}$ with highest $W_{cpu}$
  
  \ELSIF {$S_{dom} = ``N''$}
  \STATE Sort $\{W_{cand}\}$ according to $W_{net}$
  \STATE Return $W_{id}$ with highest $W_{net}$
  
  \ELSIF {$S_{dom} = ``IO''$}
  \STATE Sort $\{W_{cand}\}$ according to $W_{io}$
  \STATE Return $W_{id}$ with highest $W_{io}$  
  \ENDIF
\end{comment}

  \ELSE
  \STATE Sort $\sum_{i=0}^{i=q} r_i / m$ for $w_{id} \in W_{cand}$
  \STATE Return $w_{id}$ with highest average available resource
  
\ENDIF

\end{algorithmic}
\caption{Container Placement on Managers}
\label{alg:initial}
\end{algorithm}



\subsection{Migrating a Container}
In a Swarmkit cluster, resource contention happens on every worker.
The Container Monitor, a module of \sol, that runs on each worker node records resource usages of all hosting containers.
In addition, the worker keeps tracking available resources on itself. Whenever it finds one type of 
resources is draining and becomes a bottleneck, it sends to managers a \sol~ Alert message that contains the bottleneck type and the
most costly container of this type. Upon receiving the \sol~ Alert message, the manager needs 
to migrate this container to an appropriate worker and kill it on the worker to release the resources.

Algorithm~\ref{alg:migrate} presents the procedure to process an alert message from $w_i$.
It first builds a candidate set $W_{cand}$, which includes all running workers expect $w_i$ that sends the alert (line 1).
Then, the manager extracts the resource type, $r_i$ that causes the bottleneck and finds the corresponding $S_{id}$ for the $C_{id}$ (lines 2-4).
With $W_{cand}$ and $S_{id}$, the algorithm can decide whether this $S_{id}$ is a global service (line 5).
If $S_{id}$ is a global service and it is in the known service set, $\{KS\}$, the algorithm returns $w_{id}$ that is included the $W_{cand}$, 
with highest available $r_{S_{DOM}}$.
On the other hand, it returns $w_{id}$ with highest available $r_i$ if $S_{id}$ is not in $\{KS\}$ and $S_{DOM}$ is unknown (lines 6-12).
When $S_{id}$ is not a global service, we want to increase the reliability of $S_{id}$ by placing its containers to different workers as much as possible.
In this situation, we have a similar process expect a different $W_{cand}$, where $W_{cand}$  is all running
workers that do not hosting any containers for $S_{id}$ (lines 13 - 23).



\begin{algorithm}[ht]
\begin{algorithmic}[1]

\STATE $\{W_{cand}\}$ = All running workers expect $w_i$;
\STATE {\bf Function ReceiveAlertMsg($C_{id}$)}
\STATE Extract the bottleneck type $r_i$
\STATE Find corresponding $S_{id}$ for $C_{id}$


\IF {$\forall w_{id} \in W_{cand} \rightarrow S_{id} \in w_{id}$}

  \IF {$S_{id} \in \{KS\}$}
  \STATE $S_{DOM} = DOM(S_{id})$
  
%  \IF {$S_{DOM} \neq r_i$}
%  \STATE Return Restart the container on $w_i$
%  \ENDIF
  
\STATE Sort $W_{cand}$ according to $r_{S_{DOM}}$
\STATE Return $w_{id}$ with highest $r_{S_{DOM}}$

\ELSE
%\STATE $\forall w_{id} \in W_{cand}$, Remove $w_{id}$ from $W_{cand}$
\STATE Sort $W_{cand}$ according to $r_i$
\STATE Return $w_{id}$ with highest $r_i$

\ENDIF

  \ELSE
  \FOR {$ w_{id} \in W_{cand}$}
  \IF {$S_{id} \in w_{id}$}
  \STATE Remove $w_{id}$ from $W_{cand}$
  \ENDIF
  \ENDFOR
%  \STATE Sort $W_{cand}$ according to $r_i$
%  \STATE Return $W_{id}$ with highest available resource type $r_i$
  
\IF {$S_{id} \in \{KS\}$}
  \STATE $S_{DOM} = DOM(S_{id})$
  
%  \IF {$S_{DOM} \neq r_i$}
%  \STATE Return Restart the container on $w_i$
%  \ENDIF
  
\STATE Sort $W_{cand}$ according to $r_{S_{DOM}}$
\STATE Return $w_{id}$ with highest $r_{S_{DOM}}$

\ELSE
%\STATE $\forall w_{id} \in W_{cand}$, Remove $w_{id}$ from $W_{cand}$
\STATE Sort $W_{cand}$ according to $r_i$
\STATE Return $w_{id}$ with highest $r_i$

\ENDIF
  
\ENDIF



\end{algorithmic}
\caption{Process DRAP Alert Message from $w_i$}
\label{alg:migrate}
\end{algorithm}

